Self-similar groups and holomorphic dynamics: Renormalization, integrability, and spectrum

In this paper, we explore the spectral measures of the Laplacian on Schreier graphs for several self-similar groups (the Grigorchuk, Lamplighter, and Hanoi groups) from the dynamical and algebro-geometric viewpoints. For these graphs, classical Schur renormalization transformations act on appropriate spectral parameters as rational maps in two variables. We show that the spectra in question can be interpreted as asymptotic distributions of slices by a line of iterated pullbacks of certain algebraic curves under the corresponding rational maps (leading us to a notion of a spectral current). We follow up with a dynamical criterion for discreteness of the spectrum. In case of discrete spectrum, the precise rate of convergence of finite-scale approximands to the limiting spectral measure is given. For the three groups under consideration, the corresponding rational maps happen to be fibered over polynomials in one variable. We reveal the algebro-geometric nature of this integrability phenomenon.

==> groups.tex <==
\section{Self-similar groups and their spectrum}

\subsection{Definition}




\section{Invariant pencils for the renormalization transformations}


In this section, we explain how to find an invariant pencil for the renormalization transformations. 
Take $M (\lambda, \mu,w) \in \C[\lambda,\mu,w][G]$ a renormalizable pencil of operator and $\varphi : \C[G] \to \M_2(\C[G])$ a morphism of algebra.  
There exists a rational map $F : \P^2 \dashrightarrow \P^2$ such that:
\begin{equation*}
S_1 \varphi(M(\lambda, \mu,w)) = \bL(F(\lambda,\mu,w)).
\end{equation*}

First suppose we know that the renormalization transformation $F$ preserves a fibration, i.e that $F$ is semi-conjugated to a map on a Riemann surface $C$ via $\varphi : \P^2 \dashrightarrow C$. 
Then the fibers of $\varphi$ are mapped to other fibers of $\varphi$ by $F$ and form a family of (complex) curves of a certain degree $d$ parametrized by $C$, i.e  a pencil of curves of degree $d$  in $\P^2$. However, Bezout's theorem asserts that any two fibers of $\varphi$ intersect at $d^2$ points. The common intersection of all fibers is called the \textbf{base locus} of the pencil induced by $\varphi$. 
If we blow up the base locus of this pencil, the fibers of $\varphi$ become disjoint on the exceptional set, so each exceptional divisor is transversal to the pencil. 
However, general transversal remain transversal by the action of $F^n$ and hence cannot be collapsed. 
\medskip

In our case, we show that the base locus of an invariant pencil must be contained in the indeterminacy locus of $F$ or equivalently in the set of points where the Schur transformation is not defined. 

\begin{lem} Suppose $F$ is semi-conjugated via $\varphi : \P^2 \dashrightarrow C $ where $C$ is a projective curve.
Then a point $p$ in the base locus of the pencil induced by $\varphi$ is either regular for all iterate $F^n$ and periodic or contained in the indeterminacy locus of an iterate $F^n$.
\end{lem}


\begin{proof} Take a point $p$ in the base locus of $\varphi$. By definition, it belongs to all fibers of $\varphi$. Then $\varphi (F(p))$ takes infinitely many values. This occurs in only two situations, either $p$ is an indeterminacy point of $F$ or $p$ is regular and $F(p)$ belongs to the base locus of $\varphi$. We reiterate the previous argument to $F(p)$ and conclude as the base locus of $\varphi$ is finite.
\end{proof}



The above lemma provides good candidates for the base locus of an invariant pencil. The base locus of the pencil is contained in the regular periodic points and the indeterminacy locus. 
We shall also exclude all points $p$ which are indeterminate for $F$ but not for an iterate $F^n$. 

